Mlinear: Rethink the Linear Model for Time-series Forecasting

Recently, significant advancements have been made in time-series forecasting research, with an increasing focus on analyzing the nature of time-series data, e.g, channel-independence (CI) and channel-dependence (CD), rather than solely focusing on designing sophisticated forecasting models. However, current research has primarily focused on either CI or CD in isolation, and the challenge of effectively combining these two opposing properties to achieve a synergistic effect remains an unresolved issue. In this paper, we carefully examine the opposing properties of CI and CD, and raise a practical question that has not been effectively answered, e.g.,"How to effectively mix the CI and CD properties of time series to achieve better predictive performance?" To answer this question, we propose Mlinear (MIX-Linear), a simple yet effective method based mainly on linear layers. The design philosophy of Mlinear mainly includes two aspects:(1) dynamically tuning the CI and CD properties based on the time semantics of different input time series, and (2) providing deep supervision to adjust the individual performance of the "CI predictor" and "CD predictor". In addition, empirically, we introduce a new loss function that significantly outperforms the widely used mean squared error (MSE) on multiple datasets. Experiments on time-series datasets covering multiple fields and widely used have demonstrated the superiority of our method over PatchTST which is the lateset Transformer-based method in terms of the MSE and MAE metrics on 7 datasets with identical sequence inputs (336 or 512). Specifically, our method significantly outperforms PatchTST with a ratio of 21:3 at 336 sequence length input and 29:10 at 512 sequence length input. Additionally, our approach has a 10 $\times$ efficiency advantage at the unit level, taking into account both training and inference times.

==> abstract.tex <==
\begin{abstract}
Predicting multi-variate time series over a long future horizon is a research area that has practical applications in various domains such as electric power consumption and stock prediction. Transformer-based methods have achieved significantly better prediction performance than traditional statistical, RNN, and TCN methods, leveraging their acclaimed global modeling capability. However, most past methods have relied on inter-variable dependencies, and their prediction performance improvements often stem from self-attention mechanism enhancements and advanced deep learning techniques. Recent research suggests that discarding variable dependency assumptions and utilizing variable independence hypotheses for long-term prediction can significantly improve performance. Nevertheless, a thorough investigation into variable dependency and independence has not been adequately explored. 
%
In this paper, we explore the effective utilization of variable dependency and independence to achieve a synergistic effect, as exemplified by the popular saying ``Two heads are better than one". 
%
Specifically, we first explore the problem of joint prediction of variable independence and dependency using fixed learnable parameters. Then, we dynamically adjust variable independence and dependency features based on the temporal semantics of different input sequences. Due to the low-dimensional and high-information density characteristics of time series data, too many parameters can lead to overfitting. Therefore, we propose a deep supervision method for variable independence and dependency to supervise functionally diverse modules at different levels. Finally, we provide a loss function that outperforms current MAE and MSE to optimize the prediction model. Empirical results demonstrate that our method outperforms current state-of-the-art approaches on multiple well-established datasets.
\end{abstract}

==> approaches.tex <==
\section{Methodology}
\label{sec:approaches}
\vspace{-0.2cm}
\subsection{How is top-u $\mathbf{Q}$ calculated?}\label{how}
The canonical self-attention mechanism introduced in Transformer~\cite{vaswani2017attention} is defined by a set of tuple inputs, namely query, key, and value, that execute a scaled dot-product operation denoted as as 
\begin{equation}
\mathcal{A}(\mathbf{Q}, \mathbf{K}, \mathbf{V})= \operatorname{Softmax}\left(\mathbf{Q K}^{\top} / \sqrt{d}\right) \mathbf{V} 
\end{equation}
where $\mathbf{Q} \in \mathbb{R}^{L_Q \times d}, \mathbf{K} \in \mathbb{R}^{L_K \times d}$, $\mathbf{V} \in \mathbb{R}^{L_V \times d}$ and $d$ is the input dimension~\cite{zhou2021informer}.

%
The canonical self-attention is conventionally known for its quadratic time complexity which demands high computing resources. The \informer ~\cite{zhou2021informer} solves this problem using a KL-divergence-based approach that selects the Top-$u$ $\mathbf{Q}$ for computing the self-attention score. This method significantly enhances overall computing efficiency.
%
However, upon careful examination of the operational process of the \informer compared to the Transformer, see Fig.~\ref{Explain1}, it becomes apparent that the former has a distinguishing feature of selecting $\mathbf{K}$. Consequently, the \informer needs to perform a calculation each time to determine the positions of Top-$u$ $\mathbf{Q}$.
%
This, in turn, naturally raises a question: \textit{Is it possible to determine the position of the Top-$u$ Q in advance to avoid the need for extra calculations?}
%
To answer this question, we conducted extensive experiments and detailed analysis of Top-$u$ $\mathbf{Q}$.
\subsection{Investigate the Top-$u$ distribution explicitly}\label{distribution}
Although there has been no detailed investigation on the positioning of a single Top-$u$ $\mathbf{Q}$ in the family of formers in the time-series forecasting community~\cite{zhou2021informer}~\cite{kitaev2020reformer}~\cite{wang2020linformer}, similar research has been conducted in the computer vision community, which has directly inspired our work.
%
In Vision Transformer (ViT)~\cite{dosovitskiy2020image}, they discovered how the attention span between pixels in an image changes with the depth of the network. Fig.~\ref{fig:Four}a illustrates their findings, indicating two key observations. 
%
First, the variation in attention between adjacent layers for different pixel locations is minimal in computer vision tasks. Second, the average attention span between pixels converges to a relatively fixed range with increased depth. 
%
In response to the question above, if there is a similar pattern in Top-$u$ $\mathbf{Q}$ among each layer in a time-series prediction task, where each layer has approximately the same Top-$u$ $\mathbf{Q}$, we can use the position of the previous layer Top-$u$ $\mathbf{Q}$ to infer the position of the next layer Top-$u$ $\mathbf{Q}$ and reduce computation by one step.
%
Thus, this inspires us to explore the distribution of Top-$u$ $\mathbf{Q}$ in time-series prediction.
%
We present Fig.~\ref{fig:Four}b, which showcases our findings on ETTh1~\cite{zhou2021informer} dataset in a three-layer structure \informer model (two-layer encoder and one-layer decoder). Compared to the observations of ViT, the figure shows a substantially dissimilar result, particularly the attention positions of the second and third layers vary significantly. 
%
Considering the significant difference, utilizing the lower layer to recycle the upper Top-$u$ $\mathbf{Q}$ for reducing computational efforts may lead to a disastrous attention score (see Fig.~\ref{fig:Four}c) that will ultimately impact the predicted performance.
%
Based on this concept, we conduct a study on the Top-$u$ $\mathbf{Q}$ positions during the entire process of model training and inference. 
%
Our experimental results are presented visually in Fig.\ref{fig:Four}d. The figure displays the Top-$u$ $\mathbf{Q}$ visualized results for the complete training and inference process using ETTh1 (consisting of four rounds of iterative training and utilizing the public version of \informer). The visualized results in Fig.\ref{fig:Four}d reveal a vital finding:~\textbf{\textit{Despite parameter instability in the initial training stages, the top-u $\mathbf{Q}$ positions in the same layer remains relatively consistent when convergence is attained.}}
%
Building upon this discovery, we propose a simple yet highly effective method for reusing Top-$u$ $\mathbf{Q}$ positions. This approach significantly reduces computation overhead while preserving prediction accuracy. Detailed implementation steps are in the next section.
\begin{figure}[th]
	\centering
	\hspace*{-0.5cm}
	\subfloat [Visualization of vision Transformer attention.]{
		\includegraphics[width = 0.5\columnwidth]{fig/Explain1}
	}%
	\subfloat[Layer-wise Distribution of Top-$u$ Attention.]{
		\includegraphics[width = 0.5\columnwidth]{fig/Explain2}
	}
	\newline
	\hspace*{-0.6cm}
	\subfloat[Clear differences in the location of Top-$u$ attention between adjacent layers.]{
		\includegraphics[width = 0.5\columnwidth]{fig/Explain4}
	}
	\subfloat[Layer-wise and epoch-wise distribution of Top-$u$ attention in Informer.]{
		\includegraphics[width = 0.5\columnwidth]{fig/Explain3}
	}
	\vspace{-0.1cm}
	\caption{Visualization of Attention in vision Transformer and temporal Transformer.}
	\label{fig:Four}
	\vspace{-0.7cm}	
\end{figure}


\subsection{Detailed implementation}\label{implementation}
Our method comprises two distinct stages. The first stage involves identifying the positions of Top-$u$ $\mathbf{Q}$ during the training phase, while the second stage involves reusing the positions of Top-$u$ $\mathbf{Q}$ during the inference phase.
%

Specifically, in the training phase, we randomly select a subset of $\mathbf{K}$ and gather all $\mathbf{Q}$ from the selected subset for self-attention calculation. We then employ a measurement based on KL-divergence~\cite{zhou2021informer} to identify the $\mathbf{Q}$ with the highest self-attention score, i.e., Top-$u$, $u$ = $logL_{Q}$. 
The specific criteria used to measure attention scores are as follows:
\begin{equation}
	\bar{M}\left(\mathbf{q}_i, \mathbf{K}\right)=\max _j\left\{\frac{\mathbf{q}_i \mathbf{k}_j^{\top}}{\sqrt{d}}\right\}-\frac{1}{L_K} \sum_{j=1}^{L_K} \frac{\mathbf{q}_i \mathbf{k}_j^{\top}}{\sqrt{d}}
\end{equation}
where $\mathbf{q}_i$ and $\mathbf{k}_j$ denote each component of $\mathbf{Q}$ and $\mathbf{K}$, respectively, and $d$ denotes dimensional constant to regularize the self-attention score.
%

Subsequently, we store the computed position index of Top-$u$ $\mathbf{Q}$ and calculate its average index of positions using a particular procedure:
\begin{equation}
	\text{Top-u~Index$_{return}$} = \frac{1}{\text{Length}_{{Top-u Index}}} \sum_{i=1}^{Epoch} {\text{Top-u Index}}_i
\end{equation}   
%
where $\text{Length}_{{Top-u Index}}$ represents the total number of Top-u Index.
%

During the prediction stage, we utilize the $\text{Length}_{{Top-u Index}}$ to eliminate the need for redundant calculations in selecting Top-$u$ $\mathbf{Q}$. Instead, we can directly leverage the previous index position to identify Top-$u$ $\mathbf{Q}$ for self-attention score calculation.
%
To clarify the distinction between the inference and training stage, we outlined the entire process in Algorithm~\ref{alg}.
%
%================ALGORITHM 3====================
\begin{algorithm}[h]
	
	\small%
	%\KwIn{a CSI dataset $S$, a diffusion coefficient $d \geq 0$, a normal distribution function
		%$N$, using diffusion = $\{0,1\}$, a Positioning Neural Network $N$, a loss function $L$}
	%CSI_martrix dataset Cdataset, diffusion_coefficient = D, iterations n
	%\KwOut{the set $\mb{C}$ of clusters in $G$}
	
	\vspace{0.2cm}
	
	\ForEach{Iteration}{
		\If{Training}{
			\State{$\hat{K}\in \mathbb{R}^{\hat{L_K} \times d} =\operatorname{Sample}(K\in \mathbb{R}^{{L_K} \times d})$}
			\State{$Index_{Top-u}=\operatorname{Top-u}(\hat{K}\cdot Q)$ }
			\State{$\operatorname{Memory}(Index_{Top-u})$}
			\State{$\hat{Q}\in \mathbb{R}^{\hat{L_Q} \times d}=Q[Index_{Top-u}]$}
			\State{$Attention\in \mathbb{R}^{{L_{\hat{Q}}} \times{L_K} }=\hat{Q}\cdot K$}
			\State{$Attention\in \mathbb{R}^{{L_{{Q}}} \times{L_K} }=\operatorname{Fill}(Attention\in \mathbb{R}^{{L_{\hat{Q}}} \times{L_K} })$}
			%\State{$Attention\in \mathbb{R}^{{L_{{Q}}} \times{L_K} }=\operatorname{Fill}(Attention\in \mathbb{R}^{{L_{\hat{Q}}} \times{L_K} )$}}
		}
		\If{Predict}{
			
			\State{$Index_{Top-u}=\operatorname{Return}(\operatorname{Memory}(Index_{Top-u}))$ }
			
			\State{$\hat{Q}\in \mathbb{R}^{\hat{L_Q} \times d}=Q[Index_{Top-u}]$}
			\State{$Attention\in \mathbb{R}^{{L_{\hat{Q}}} \times{L_K} }=\hat{Q}\cdot K$}
			\State{$Attention\in \mathbb{R}^{{L_{{Q}}} \times{L_K} }=\operatorname{Fill}(Attention\in \mathbb{R}^{{L_{\hat{Q}}} \times{L_K} })$}
			
		}
	}
	\State{\textbf{until} the end}
	\caption{Detailed steps.}
	\label{alg}
\end{algorithm}

%================ALGORITHM 3====================
%
To ensure that the effectiveness of our proposed \Prophetattention is fully validated, we incorporate it into \informer, and tested it on four widely used datasets.




==> command.tex <==
\newcounter{example}[section]
\renewcommand{\theexample}{\nthesection.\arabic{example}}
\newenvironment{example}{
     \refstepcounter{example}
     {\vspace{1ex} \sc  Example  \theexample:}}{
     \eot\vspace{1ex}} %\hspace*{\fill}\vspace*{1ex}}

\newcounter{definition}[section]
\renewcommand{\thedefinition}{\nthesection.\arabic{definition}}
\newenvironment{definition}{
     \refstepcounter{definition}
     {\vspace{1ex} \sc  Definition  \thedefinition:}}{
	\vspace{1ex}} %\hspace*{\fill}\vspace*{1ex}}

\newcounter{theorem}[section]
\renewcommand{\thetheorem}{\nthesection.\arabic{theorem}}
\newenvironment{theorem}{\begin{em}
        \refstepcounter{theorem}
        {\vspace{1ex} \sc  Theorem  \thetheorem:}}{
		\end{em}\vspace{1ex}} %\hspace*{\fill}\vspace*{1ex}}

\newcounter{lemma}[section]
\renewcommand{\thelemma}{\nthesection.\arabic{lemma}}
\newenvironment{lemma}{\begin{em}
        \refstepcounter{lemma}
        {\vspace{1ex} \sc Lemma \thelemma:}}{
		\end{em}\vspace{1ex}} %\hspace*{\fill}\vspace*{1ex}}

\newcommand{\proofsketch}{\noindent{\sc Proof Sketch: }}
\newcommand{\myproof}{\noindent{\sc Proof: }}

\newcommand{\nthesection}{\arabic{section}}

% End of proof
\newcommand{\eot}{\hspace*{\fill}\mbox{$\Box$}}
% \newcommand{\eop}{\hspace*{\fill}\mbox{$\blacksquare$}}
\newcommand{\eop}{\hspace*{\fill}\mbox{$\Box$}\vspace*{1ex}}

% Small Title
\newcommand{\stitle}[1]{\vspace{1ex} \noindent{\bf #1}}

\newcommand{\kw}[1]{{\ensuremath {\mathsf{#1}}}\xspace}

\newcommand{\la}{\leftarrow}

\newcommand{\cfig}{Figure~}
\newcommand{\ctab}{Table~}
\newcommand{\csec}{Section~}
\newcommand{\cdef}{Definition~}
\newcommand{\calg}{Algorithm~}
\newcommand{\cthm}{Theorem~}
\newcommand{\clem}{Lemma~}
\newcommand{\cequ}[1]{Equation~(#1)}

\newcommand{\ie}{{\it i.e.}}
\newcommand{\eg}{{\it e.g.}}


==> conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
In this paper, we conduct a detailed study on the long-tailed distribution of self-attention score and discover a regularity in which the active attention positions are relatively fixed. Based on this finding, we propose a novel self-attention calculation method that can reuse the active attention positions. 
%
Extensive experiments on the latest model of sparse attention mechanism, \informer, by embedding our proposed \Prophetattention, demonstrate that our method not only improves prediction accuracy but also significantly enhances prediction speed.
%
%In future work, it is of interest to explore different attention operations and to apply this approach to computer vision, natural language processing and other fields.


==> experiments.tex <==
\section{Experiments}
\label{sec:exp}
\vspace{-0.3cm}
\subsection{Experimental Setup}\label{sec:setup}
\subsubsection{Dataset}
We use four datasets in our experiments, \ie, {\em Electricity Transformer Temperature} (\etth, \etthh, \ettm) and {\em Weather} (\wth).
%
\etth and \etthh both consist of six-variable time series that record power load features every hour.
% 
\ettm records data every 15 minutes, but it is similar to \etth and \etthh.
%
\wth provides climatological data for almost 1,600 locations in the United States from 2010 to 2013. The data is taken hourly and consists of 11 climate features and the target variable `wet bulb'. 
%
To ensure a fair comparison with \informer~\cite{zhou2021informer}, our train/validation/test data covers 12/4/4 months for \etth, \etthh, and \ettm, and 28/10/10 months for \wth.
%
\subsubsection{Settings}
To train our model, we adopt the Adam~\cite{kingma2014adam} optimizer with an initial learning rate of 1$e^{-4}$ which is gradually reduced by a factor of 0.5 each epoch. We employ a batch size of 32 and perform early stopping with a patience of 3, stopping the training process after a maximum of 8 epochs.
%
Notably, our experimental settings are kept identical to those of \informer~\cite{zhou2021informer} to ensure a fair comparison. All models are trained/tested using a single NVIDIA V100 GPU.
%
\begin{table*}[t]
	
	\centering%把表居中
	\begin{center}
		\resizebox{\columnwidth}{!}{
			\begin{tabular}{c|c|cc|cc|cc|cc|cc|cc|cc|cc}
				
				\toprule
				\multicolumn{2}{c|}{Methods} &
				\multicolumn{2}{c|}{Ours} &
				\multicolumn{2}{c|}{Informer} &
				\multicolumn{2}{c|}{LogTrans} &
				\multicolumn{2}{c|}{Reformer} &
				\multicolumn{2}{c|}{LSTMa} &
				\multicolumn{2}{c|}{DeepAR} &
				\multicolumn{2}{c|}{ARIMA} &
				\multicolumn{2}{c}{Prophet} \\
				\midrule
				\multicolumn{2}{c|}{Metric}   & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE \\
				\midrule
				\multirow{5}{*}{\rotatebox{90}{\large{ETTh1}}} 
				& 24 & \textbf{0.088}&\textbf{0.237}&0.098&0.247&0.103&0.259&0.222&0.389&0.114&0.272&0.107&0.280&0.108&0.284&0.115&0.275\\
				
				& 48  & \textbf{0.125}&\textbf{0.315}&0.158&0.319&0.167&0.328&0.284&0.445&0.193&0.358&0.162&0.327&0.175&0.424&0.168&0.330 \\
				
				
				& 168 & \textbf{0.151}&\textbf{0.272}&0.183&0.346&0.207&0.375&1.522&1.191&0.236&0.392&0.239&0.422&0.396&0.504&
				1.224&0.763\\
				
				
				& 336 & \textbf{0.118}&\textbf{0.293}&0.222&0.387&0.230&0.398&1.860&1.124&0.590&0.698&0.445&0.552&0.468&0.593&1.549&1.820\\
				
				
				
				& 720 & \textbf{0.137}&\textbf{0.281}&0.269&0.435&0.273&0.463&2.112&1.436&0.683&0.768&0.658&0.707&0.659&0.766&2.735&3.253\\
				\midrule
				\multirow{5}{*}{\rotatebox{90}{\large{ETTh2}}} 
				
				& 24  &\textbf{0.083}&\textbf{0.222}&0.093&0.240&0.102&0.255&0.263&0.437&0.155&0.307&0.098&0.263&3.554&0.445&0.199&0.381\\
				
				
				
				& 48  &\textbf{0.152}&\textbf{0.307}&0.155&0.314&0.169&0.348&0.458&0.545&0.190&0.348&0.163&0.341&3.190&0.474&0.304&0.462\\
				
				
				& 168 &{0.286}&{0.430}&\textbf{0.232}&\textbf{0.389}&0.246&0.422&1.029&0.579&0.385&0.514&0.255&0.414&2.800&0.595&2.145&1.068\\
				
				
				
				
				& 336 &0.290&0.436&\textbf{0.263}&\textbf{0.417}&0.267&0.437&1.668&1.228&0.558&0.606&0.604&0.607&2.753&0.738&2.096&2.543\\
				
				
				
				
				& 720 &\textbf{0.261}&\textbf{0.416}&0.277&0.431&0.303&0.493&2.030&1.721&0.640&0.681&0.429&0.580&2.878&1.044&3.355&4.664\\
				\midrule
				\multirow{5}{*}{\rotatebox{90}{\large{ETTm1}}} 
				
				
				& 24  &\textbf{0.022}&\textbf{0.114}&0.030&0.137&0.065&0.202&0.095&0.228&0.121&0.233&0.091&0.243&0.090&0.206&0.120&0.290\\
				
				
				& 48  &\textbf{0.046}&\textbf{0.166}&0.069&0.203&0.078&0.220&0.249&0.390&0.305&0.411&0.219&0.362&0.179&0.306&0.133&0.305\\
				
				
				& 96 &\textbf{0.168}&\textbf{0.347}&0.194&0.372&0.199&0.386&0.920&0.767&0.287&0.420&0.364&0.496&
				0.272&0.399&0.194&0.396\\
				
				
				& 228 &\textbf{0.292}&\textbf{0.465}&0.401&0.554&0.411&0.572&1.108&1.245&0.524&0.584&0.948&0.795&0.462&0.558&0.452&0.574\\
				& 672 &\textbf{0.356}&\textbf{0.522}&0.512&0.644&0.598&0.702&1.793&1.528&1.064&0.873&2.437&1.352&0.639&0.697&2.747&1.174\\
				
				
				\midrule
				\multirow{5}{*}{\rotatebox{90}{\large{Weather}}} 
				& 24  &\textbf{0.113}&\textbf{0.246}&0.117&0.251&0.136&0.279&0.231&0.401&0.131&0.254&0.128&0.274&0.219&0.355&0.302&0.433\\
				
				
				& 48  &0.191&0.326&\textbf{0.178}&\textbf{0.318}&0.206&0.356&0.328&0.423&0.190&0.334&0.203&0.353&0.273&0.409&0.445&0.536\\
				
				
				& 168 &\textbf{0.256}&\textbf{0.381}&0.266&0.398&0.309&0.439&0.654&0.634&0.341&0.448&0.293&0.451&0.503&0.599&2.441&1.142\\
				
				
				
				& 336 &\textbf{0.290}&\textbf{0.407}&0.297&0.416&0.359&0.484&1.792&1.093&0.456&0.554&0.585&0.644&0.728&0.730&1.987&2.468\\
				
				& 720 &\textbf{0.326}&\textbf{0.426}&0.359&0.466&0.388&0.499&2.087&1.534&0.866&0.809&0.499&0.596&1.062&0.943&3.859&1.144\\
				\midrule
				\multicolumn{2}{c|}{Count} &
				\multicolumn{2}{c|}{34} &
				\multicolumn{2}{c|}{6} &
				\multicolumn{2}{c|}{0} &
				\multicolumn{2}{c|}{0} &
				\multicolumn{2}{c|}{0} &
				\multicolumn{2}{c|}{0} &
				\multicolumn{2}{c|}{0} &
				\multicolumn{2}{c}{0} \\
				\midrule
		\end{tabular}}
		\caption{Univariate long sequence time-series forecasting results on four datasets (five cases).}
		\label{single}
	\end{center}
\end{table*}



\begin{table*}[t]
	
	\centering%把表居中
	\begin{center}
		\resizebox{\columnwidth}{!}{
			\begin{tabular}{c|c|cc|cc|cc|cc|cc|cc}
				
				\toprule
				\multicolumn{2}{c|}{Methods} &
				\multicolumn{2}{c|}{Ours} &
				\multicolumn{2}{c|}{Informer} &
				\multicolumn{2}{c|}{LogTrans} &
				\multicolumn{2}{c|}{Reformer} &
				\multicolumn{2}{c|}{LSTMa} &
				\multicolumn{2}{c}{LSTnet} 
				\\
				\midrule
				\multicolumn{2}{c|}{Metric}   & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE & MSE & MAE  \\
				\midrule
				\multirow{5}{*}{\rotatebox{90}{\large{ETTh1}}} 
				& 24 & \textbf{0.560}&\textbf{0.546}&0.577&0.549&0.686&0.604&0.991&0.754&0.650&0.624&1.293&0.901\\
				& 48  & \textbf{0.683}&\textbf{0.623}&0.685&0.625&0.766&0.757&1.313&0.906&0.702&0.675&1.456&0.960 \\
				& 168 & 1.082&0.827&\textbf{0.931}&\textbf{0.752}&1.002&0.846&1.824&1.138&1.212&0.867&1.997&1.214\\				
				& 336 & 1.233&0.887&\textbf{1.128}&\textbf{0.873}&1.362&0.952&2.117&1.280&1.424&0.994&2.655&1.369\\
				& 720 & 1.380&0.950&\textbf{1.215}&\textbf{0.896}&1.397&1.291&2.415&1.520&1.960&1.322&2.143&1.380\\
				\midrule
				\multirow{5}{*}{\rotatebox{90}{\large{ETTh2}}} 

				& 24  &\textbf{0.550}&\textbf{0.576}&0.720&0.665&0.828&0.750&1.531&1.613&1.143&0.813&2.742&1.457\\
				
				
				
				& 48  &\textbf{1.314}&\textbf{0.894}&1.457&1.001&1.806&1.034&1.871&1.735&1.671&1.221&3.567&1.687\\
				& 168 &4.814&1.862&\textbf{3.489}&\textbf{1.515}&4.070&1.681&4.660&1.846&4.117&1.674&3.242&2.513\\
				& 336 &\textbf{2.448}&\textbf{1.280}&2.723&1.340&3.875&1.763&4.028&1.688&3.434&1.549&2.544&2.591\\
			
				& 720 &\textbf{3.384}&1.604&3.467&\textbf{1.473}&3.913&1.552&5.381&2.015&3.963&1.788&4.625&3.709\\
				\midrule
				\multirow{5}{*}{\rotatebox{90}{\large{ETTm1}}} 
				
				
				& 24 &\textbf{0.317}&\textbf{0.369}&0.323&\textbf{0.369}&0.419&0.412&0.724&0.607&0.621&0.629&1.968&1.170\\
				
				& 48 &\textbf{0.476}&\textbf{0.472}&0.494&0.503&0.507&0.583&1.098&0.777&1.392&0.939&1.999&1.215\\
				
				& 96 &\textbf{0.511}&\textbf{0.511}&0.678&0.614&0.768&0.792&1.433&0.945&1.339&0.913&2.762&1.542\\
				
				& 228 &\textbf{0.922}&\textbf{0.746}&1.056&0.786&1.462&1.320&1.820&1.094&1.740&1.124&1.257&2.076\\
				& 672 &\textbf{0.953}&\textbf{0.770}&1.192&0.926&1.669&1.461&2.187&1.232&2.736&1.555&1.917&2.941\\
				
				\midrule
				\multirow{5}{*}{\rotatebox{90}{\large{Weather}}} 
				& 24  &\textbf{0.330}&\textbf{0.380}&0.335&0.381&0.435&0.477&0.655&0.583&0.546&0.570&0.615&0.545\\
				
				
				& 48  &\textbf{0.383}&\textbf{0.422}&0.395&0.459&0.426&0.495&0.729&0.666&0.829&0.677&0.660&0.589\\
				
				
				
				
				& 168 &\textbf{0.603}&{0.571}&0.608&\textbf{0.567}&0.727&0.671&1.318&0.855&1.038&0.835&0.748&0.647\\
			
				& 336 &\textbf{0.681}&\textbf{0.620}&0.702&\textbf{0.620}&0.754&0.670&1.930&1.167&1.657&1.059&0.782&0.683\\
				
				& 720 &\textbf{0.667}&\textbf{0.608}&0.831&0.731&0.885&0.773&2.726&1.575&1.536&1.109&0.851&0.757\\
				\midrule
				\multicolumn{2}{c|}{Count} &
				\multicolumn{2}{c|}{30} &
				\multicolumn{2}{c|}{12} &
				\multicolumn{2}{c|}{0} &
				\multicolumn{2}{c|}{0} &
				\multicolumn{2}{c|}{0} &
				\multicolumn{2}{c}{0}  \\
				\midrule
		\end{tabular}}
		\caption{Multivariate long sequence time-series forecasting results on four datasets (five cases).}
		\label{multi}
	\end{center}
\end{table*}

\subsection{Performance Comparison and Analysis}
To incorporate our proposed \ProphetAttention, we replaced the self-attention layer in \informer. We then compared the obtained new model against \informer~\cite{zhou2021informer}, \reformer\cite{kitaev2020reformer}, \lstma~\cite{bahdanau2014neural}, \logtrans~\cite{li2019enhancing}, \deepar~\cite{salinas2020deepar}, \arima~\cite{ariyo2014stock}, and \prophet~\cite{taylor2018forecasting}. Table~\ref{single} and Table~\ref{multi} present the comprehensive accuracy results, with the best performing models highlighted in bold.
%
From Table~\ref{single}, it can be seen that our model can achieve high prediction performance under the setting of univariate prediction. 
%
It obtain the best results in 34 out of 40 comparison indicators, while \informer obtain the best results in 6 indicators. Especially when the prediction length is extended, our model achieves better prediction performance compared to \informer. For example, at a prediction length of 720 steps in ETTh1, our model reduces the prediction MSE from 0.269 to 0.137, which is a decrease of approximately 49.44\% compared to Informer. 
%
From Table 2, it can be observed that prophetattention also achieved the best prediction performance under the setting of multi-variable prediction, obtaining the best results in 30 out of 40 comparison indicators, while informer obtain the best results in 12 indicators. 
%
It is worth noting that the suboptimal results of \ProphetAttention are mainly concentrate in the \etth and \etthh datasets, due to the coarse feature granularity of these two datasets (recording intervals of 1 hour). 
%
The coarse-grained records lead to small differences in numerical values between different points, resulting in not enough distinction in self-attention score. 
%
Although \ProphetAttention do not show significant performance improvements in this situation, considering the significant improvement in prediction efficiency and the comprehensive consideration of the four datasets, it can be verified that \ProphetAttention is effective.
%
In addition, we conduct an efficiency analysis of proposed \ProphetAttention, and considering that Informer achieved the highest efficiency through sparse attention, our efficiency comparison is mainly compared with Informer.
From Figure~\ref{time}, it can be observed that the prediction time of our model slightly increases with the increase of the prediction horizon, indicating that our model is capable of maintaining high prediction efficiency in handling longer time series. In contrast, the prediction time of the Informer model dramatically increases with the increase of the prediction horizon, possibly due to the complexity of the model causing bottlenecks in handling long time series. Results show that our model improves the prediction efficiency compared to the Informer model by approximately 17\% - 26\% across all prediction horizons.
%\subsection{Does our method work only on sparse attention?}


\begin{comment}
	
	\begin{figure}[!t]
		\centering
		\includegraphics[width=3in,height=1.6in]{fig/attention}
		\caption{}
		\label{Attention}
		%\vspace{-0.5cm}
	\end{figure}
	内容...
\end{comment}



\begin{figure*}[t]
	\vspace{-0.3cm}
	\centering
	\includegraphics[width=1.0\columnwidth]{fig/V100time}
	%\vspace{-0.3cm}
	\caption{Comparison of Inference Time}
	\vspace{-0.7cm}
	\label{time}
\end{figure*}

==> introduction.tex <==
\section{Introduction}
\label{sec:introduction}
\vspace{-0.3cm}
Transformer has led a revolution in time-series analysis, owing to its exceptional aptitude in modeling sequential data with long-term dependencies. 
%
Its supremacy over conventional approachs~\cite{huang2023intrinsic}~\cite{money2022online}~\cite{rahman2022comprehensive}, conventional convolution neural networks~(CNNs)~\cite{hewage2020temporal}~\cite{zheng2022denoising} and recurrent neural networks (RNNs)~\cite{luo2020dual}~\cite{tokgoz2018rnn} can be attributed to the employment of self-attention mechanism that enables the efficient gathering of information from every time step while overcoming the issue of vanishing gradients.
%

Given the remarkable effectiveness of Transformer~\cite{vaswani2017attention}, many subsequent improvement works have been proposed, particularly in the application area of time-series analysis and prediction, such as \informer~\cite{zhou2021informer}, \reformer~\cite{kitaev2020reformer}, \linformer~\cite{wang2020linformer}, \sparseformer~\cite{child2019generating}. 
%
These researchs have made various improvements and optimizations to Transformer, enriching the `Transformer family' with many excellent members and covering many practical applications~\cite{gong2022load}~\cite{lee2019unified}~\cite{jiang2022very}. 
%
It is worth noting that among the various techniques proposed in these works, the most impressive one is the unique self-attention mechanism they proposed.
%
For example, \linformer~\cite{wang2020linformer} uses linear mapping to reduce the length of $\mathbf{Q}$ and $\mathbf{K}$, limiting the time complexity of self-attention to $O(n)$. 
%
\sparseformer~\cite{child2019generating} discovers the sparsity of self-attention and uses a few attention points with larger weights to provide a more focused attention score. 
%
\informer~\cite{zhou2021informer} defines a measurement based on KL-divergence and uses a small amount of computation to obtain Top-$u$ $\mathbf{Q}$ with a high self-attention score, followed by dot product operations with Top-$u$ $\mathbf{Q}$ and $\mathbf{K}$ to obtain the self-attention score. 
%
Although these studies have all noticed the sparse distribution in self-attention and have achieved significant results by exploiting this phenomenon, it is evident that they have only focused on the overall distribution of attention and have not finely considered the scores of individual attention, leaving much room for improvement.
%
For instance, \sparseformer only heuristically constrains each sequence point to be related to only $k$ surrounding points and itself. There has been no theoretical analysis or empirical discussion of this approach, only effectiveness assessments from a performance perspective. 
%
\informer selects active Top-$u$ $\mathbf{Q}$ from the overall $\mathbf{Q}$ for self-attention calculation, without any further analysis of this Top-$u$ $\mathbf{Q}$, for instance, \textit{what are the distribution patterns of the Top-$u$ $\mathbf{Q}$? Do the Top-$u$ $\mathbf{Q}$ in different attention layers have the same distribution?}

%
Following the latest research of the `Transformer family', we conducted a detailed study of the specific distribution of active Top-$u$ attention and derived two important conclusions: 
(1) The position of Top-$u$ attention in a single attention layer is relatively fixed after stable training. 
(2) The Top-$u$ attention in different attention layers has significant differences. 
%
Based on these observations, we propose a novel self-attention called \ProphetAttention. Specifically, \ProphetAttention consists of two different execution stages. 
%
In the training stage, \ProphetAttention adopts the same process for selecting Top-$u$ attention as \informer but marks the Top-$u$ attention position for different attention layers. 
%
In the prediction stage, since the Top-$u$ attention (the more popular explanation is the Top-$u$ index) has already been labeled, different attention layers use the previous position markings for attention calculation, thereby avoiding redundant Top-$u$ measurement processes. 
%
We embed \ProphetAttention into \informer and replace the sparse-attention of \informer to verify the effectiveness of \ProphetAttention. Results on four widely used datasets show that \ProphetAttention can achieve comparable performance and significantly improve the model's prediction speed.
%
In summary, our work makes the following contributions:
\begin{enumerate}
	\item We further explore the long-tail distribution of attention and identify the specific layer-wise and epoch-wise distribution patterns of attention in long-tail distributions.
	\item Based on our observations, we propose a novel self-attention mechanism called \ProphetAttention, which can reduce redundant computations of sparse attention during the prediction stage by reusing previously active attention positions.
	\item We embed \ProphetAttention into the latest sparse-attention model, \informer, to validate its effectiveness. Experiments on four widely used time-series prediction datasets demonstrate that our model outperforms all the 80 compared baselines 64 times and significantly improves the prediction efficiency.
\end{enumerate}
\begin{figure*}[t]
	\vspace{-0.3cm}
	\centering
	\includegraphics[width=1.0\columnwidth]{fig/All}
	%\vspace{-0.3cm}
	\caption{(Left) Detailed process: Informer uses self-attention score to search for active Q, and uses the active Q to calculate self-attention output. (Right) Distinct self-attention score and indistinct self-attention score.}
	\vspace{-0.7cm}
	\label{Explain1}
\end{figure*}
%

The rest of this paper is organized as follows.
%
First, we use \informer as an example to introduce how to calculate Top-$u$ $\mathbf{Q}$ in Section~\ref{how}.
%
Then, Section~\ref{distribution} shows our investigation on the specific distribution and position of Top-$u$ attention.
%
Third, Section~\ref{implementation} introduces our proposed \ProphetAttention and the implementation steps of applying it to sequence prediction.
%
In addition, Section~\ref{sec:exp} presents the detailed results of embedding \ProphetAttention into \informer and applying it to four datasets.
%
Finally, we draw several conclusions in Section~\ref{sec:conclusion}.



==> related.tex <==
\section{Related Work}
\label{sec:related}

\subsection{Short-term Forecasting with \rnns and \tcns}
The short term usually means a few dozen steps ahead. 
In this domain, there are often two types of models can good capture short-term temporal dependencies-- recurrent neural networks (\rnns) and temporal convolutions networks (\tcns).
%
Bai et al.~\cite{bai2019passenger} extract data's spatial correlations by \cnn, and use \lstm to do predict.
%
Li et al.~\cite{li2017diffusion} model time-series data as a diffusion process on a directed graph and introduce a \rnn based neural network, called Diffusion Convolutional Recurrent Neural Network for forecasting.
%
Seo et al.~\cite{seo2018structured} proposed a \rnn based deep learning neural network used for structured time-series sequence, and it can be adapted to data structured by an arbitrary graph temporal convolutions network (\tcns).
%
Ke et al.~\cite{ke2017short} simultaneously consider the spatial dependences, temporal dependences, and exogenous dependences. 
And they propose a fusion convolutional network, named ``fusion convolutional long short-term memory network'' to do forecasting. 
%
Wu et al.~\cite{wu2019graph} propose a novel neural network for spatial-temporal graph modeling. They learning node embedding to develop an adaptive dependency matrix for capture the spatial dependency in the data.
%
Cao et al.~\cite{cao2020spectral} jointly captures inter-series correlations and temporal dependencies in the spectral domain and use a graph neural network to improve the accuracy of time-series forecasting. 
Although \rnns and \tcns achieve better results in short-term domain, but limited by their models' inner defect, \eg, rely on intermediate representations ~\cite{khandelwal2018sharp}, they fall short on long-term forecasting. 

\subsection{Long-term Forecasting with Transformers}
In terms of long-term forecasting, attention based models achieve better results than \rnns and \tcns. 
People tend to think the theoretical shortest $\mathcal{O}(1)$ maximum length of network signals traveling paths or the non-recurrent structure have a work. 
%
Most recent works focus their work on improving the efficiency of \transformer's canonical attention in a macroscopic perspective. 
%
In this paper, we explore the relationship between individual attention and model ability from a more detailed perspective.
%
\reformer~\cite{kitaev2020reformer} use locality-sensitive hashing to replace dot-product attention enable the complexity reduce to $\mathcal{O}(L\cdot logL)$, performs on par with \transformer models on long sequences. 
%
\linformer~\cite{wang2020linformer} use a low-rank matrix to approximate the self-attention mechanism and reduce the complexity to $\mathcal{O}(L\cdot logL)$.
%
\funnel~\cite{dai2020funnel} reduces the computation cost by a gradual way, they compress the sequence of hidden states to a shorter one thus improves the model capacity.
%
\triformer~\cite{cirstea2022triformer} uses a patch attention with linear complexity to replace the original self-attention and introduces a triangular structure to shrink the layer sizes.
%
\informer~\cite{zhou2021informer} uses a measurement to select the active $Q$ to calculate the self-attention, and use a pooling structure to reduce the memory usage.
%
The attention's table is shown in Table~\ref{attention_table}.
%
The above work mainly focus on the efficiency of self-attention. 
They all black-box method and fail in attention detail, \eg, does not consider whether attention is positive or negative for predicting. 
%
By studying the relationship between individual attention and model ability, we propose a novel efficient attention mechanism which called dual-feedback attention with the $\mathcal{O}(L\cdot logL)$ complexity. 
It able to extract reliable attention by a white-box method. 
Next, the dependency extraction and noise elimination will make further optimizations.
%
We analyze the advantages and disadvantages of different based methods, the conclusion can be seen in Fig.~\ref{fig:fig2}.

\begin{figure}[t]
	\centering
	\hspace*{-0.5cm}
	\subfigure[]{
		\includegraphics[width = 0.47\columnwidth]{fig/RACability}
	}%
	\subfigure[]{
		\includegraphics[width = 0.47\columnwidth]{fig/RACeff}
	}
	%\vspace{-0.3cm}
	\caption{Efficiency and ability for different based methods}
	\label{fig:fig2}
	%\vspace{-0.7cm}	
\end{figure}


